Building Rome with Convex Optimization

Global bundle adjustment is made easy by depth prediction and convex optimization. We (i) propose a scaled bundle adjustment (SBA) formulation that lifts 2D keypoint measurements to 3D with learned depth, (ii) design an empirically tight convex semidfinite program (SDP) relaxation that solves SBA to certfiable global optimality, (iii) solve the SDP relaxations at extreme scale with Burer-Monteiro factorization and a CUDA-based trust-region Riemannian optimizer (dubbed XM), (iv) build a structure from motion (SfM) pipeline with XM as the optimization engine and show that XM-SfM compares favorably with existing pipelines in terms of reconstruction quality while being significantly faster, more scalable, and initialization-free.

==> sections/note.tex <==
%!TEX root = ../main.tex

\section{Note for discussion}
\label{sec:note}

\subsection{Jan 4}

\begin{itemize}
    \item Components
    \begin{enumerate}
        \item \teaser++: 3D-3D registration
        \item re\ransac: 2D-3D registration
        \item \glomap two-view filter: 3D-3D registration
    \end{enumerate}
    Finally we choose 
    \begin{enumerate}
        \item \nameshort purely as a baseline, denote by \nameshort
        \item \nameshort running for two times, denote by \xmdouble
        \item \xmdouble + re\ransac + \teaser++ as one pipline, denote by \xmdouble-T
        \item \xmdouble + \glomap two-view filter as another pipeline, denote by \xmdouble-F
    \end{enumerate}
    These three are all filters. These filter method now have the following thing we have not figured out:
    \begin{enumerate}[label={\checkmark}]
        \item \textcolor{red}{How to tune the hyper-parameters?}
        \item \textcolor{red}{It may cause the number of images decrease.}
        \item \textcolor{red}{It may make the view-graph sparse.}
    \end{enumerate}
    \item Neural rendering:
    Plan to use \colmap, seems glomap is not that stable.
    \item Breakdown plot
    \begin{enumerate}[label={\checkmark}]
        \item \textcolor{green}{Add solver time}
        \item \textcolor{green}{Remove \teaser + \ransac}
    \end{enumerate}
    \item Visualization
    \begin{enumerate}[label={\checkmark}]
        \item \textcolor{red}{Add circle rotation Visualization}
    \end{enumerate}
    \item Replica main table
    \begin{enumerate}[label={\checkmark}]
        \item \textcolor{green}{Change to median}
        \item \textcolor{green}{separate solve and propress time for glomap.}
    \end{enumerate}
    \item Suboptimality
    The math of suboptimility is here:
    For the problem with regularity term, the primal problem is:
    \begin{align}
    \min ~~&\langle C, X \rangle + Q(X)\\
    s.t. ~~&X \succ 0\\
    & \langle A_i, X \rangle = b_i, ~~\forall i
    \end{align}
    $Q(X)$ is a quadratic term defined by $Q(X) = \lambda \sum_i (X_{ii}-1)^2$. This is still a convex problem and the lagrangian is:
    \begin{align}
    L(X, y, Z) =& \langle C, X \rangle + Q(X) - \\&\sum_i y_i (\langle A_i, X \rangle - b_i) - \langle Z, X \rangle \\
    =& \langle C - \sum_i y_i A_i - Z, X \rangle + Q(X) + \sum_i y_i b_i
    \end{align}
    The KKT condition is:
    \begin{align}
    Z =& C + \nabla Q(X) - \sum_i y_i A_i \succ 0 \\
    \langle A_i, X \rangle =& b_i, ~~\forall i \\
    X \succ & 0 \\
    \langle Z, X \rangle = & 0
    \end{align}
    \red{For $Q(X) = 0$ I know to get $\inf L(X, y, Z)$  finite we need $C - \sum_i y_i A_i = Z \succ 0$. }
    Note $L$ is linear in the off-diagnol elements of $X$, and quadratic in the diagnol elements of $X$. To get the minimum finite, we need $(\nabla L)_{ij} = 0,~i\neq j$. For the diagnol elements, we need $(\nabla L)_{ij} = 0$ to get the minimal point. So together we will need $\nabla L = 0$, i.e.
    \begin{align}
    C - \sum_i y_i A_i - Z = -\nabla Q(X)
    \end{align}
    From diagnol we know $X_{ii} = -\frac{(C - \sum_i y_i A_i - Z)_{ii}}{2\lambda} + 1$. So we plug in $X$ then we get the dual problem:
    \begin{align}
    \max ~~&\sum_i b_i y_i - \frac{\sum_j (C - \sum_i y_i A_i - Z)_{jj}^2}{4\lambda} 
    \\ & + \sum_j (C - \sum_i y_i A_i - Z)_{jj} \\
    s.t. ~~&Z \succ 0\\
         ~~&(C - \sum_i y_i A_i - Z)_{ij} = 0, ~~i\neq j    
    \end{align}
    To derive the sub-optimality gap, we assume primal is feasible, then for all feasible $X$ we have:
    \begin{align}
    \langle C, X \rangle + Q(X) &\geq \langle C - \sum_i y_i A_i + \nabla Q(x) , X \rangle \\
    &+ \underbrace{\sum_i y_i b_i + Q(X) - \langle \nabla Q(X), X \rangle}_{\text{dual value}}\\
    &= \langle Z, X \rangle + p_{\text{dual}}\\
    &\geq \text{max}(0,\lambda_{\text{min}}(Z)) \text{tr}(X) + p_{\text{dual}}
    \end{align}
    then we define the sub-optimality gap as:
    \begin{align}
    p_{\text{primal}} - p_{\text{dual}} - \text{max}(0,\lambda_{\text{min}}(Z)) \text{tr}(X)
    \end{align}
\end{itemize}

\subsection{Jan 10}
\begin{itemize}
    \item Undistort images -- if it is radial camera, need to do undistortion
\end{itemize}


==> sections/related-works.tex <==
%!TEX root = ../main.tex

\section{Related Works}
\label{sec:relatedworks}

\subsection{Polynomial optimization and Moment-SOS hierarchy}
As a general modeling and optimization tool, polynomial optimization problems (POPs) are prevalent in various fields such as control~\cite{majumdar2013icra-controldedsign-sos}, perception~\cite{yang2022pami-outlierrobust-geometricperception}, and optimal transport~\cite{mula2022arxiv-momentsos-optimal-transport}. 
The celebrated Moment-SOS Hierarchy~\cite{lasserre2001siopt-global} offers a powerful tool to solve POP to global optimality asymptotically. By leveraging the duality between moment relaxation and sum-of-squares (SOS) relaxation, POP is solved by a series of monotonically growing SDPs. Under certain constraint qualification conditions~\cite{nie2023siopt-moment-momentpolynomialopt}, finite convergence can be observed~\cite{yang2022pami-outlierrobust-geometricperception,teng2023arxiv-geometricmotionplanning-liegroup}. To enhance scalability, researchers exploit various sparsity patterns, including correlative sparsity~\cite{lasserre2006msc-correlativesparse}, term sparsity~\cite{wang2021siam-tssos}, and ideal sparsity~\cite{korda2023mp-ideal-sparsity}, which significantly improves computation.

\subsection{Semidefinite programming (SDP) solvers}
For small to medium-scale general SDPs, the interior point method~\cite{helmberg1996siam-interiorpoint-sdp} is the preferred choice due to its robustness and high accuracy, with several academic and commercial solvers available~\cite{tutuncu2003mp-sdpt3-sdpsolver,sturm1999oms-sedumi-sdpsolver,aps2019ugrm-mosek-sdpsolver}. As SDP size increases, first-order methods, particularly ADMM-style algorithms~\cite{wen2010mp-admmsdp,chen2017mp-sgsadmm,li2018mp-sgs-ccqp,chen2021mp-alm-admm-equivalence}, become more popular due to their affordable per-iteration time and memory cost. Among these, sGS-ADMM~\cite{chen2017mp-sgsadmm,li2018mp-sgs-ccqp} demonstrates superior empirical performance. Several academic first-order SDP solvers are available~\cite{odonoghue2023-scs-sdpsolver,zheng2017ifac-cdcs-sdpsolver,yang2015mp-sdpnalplus-sdpsolver}. In real-world applications~\cite{yang2022pami-outlierrobust-geometricperception,teng2023arxiv-geometricmotionplanning-liegroup}, many SDPs exhibit a low-rank property, prompting the development of specialized algorithms~\cite{burer2003springer-bm,tang2023arxiv-feasible-lowranksdp} and solvers~\cite{yang2023mp-stride,wang2023arxiv-manisdp}. However, these algorithms often underperform for large-scale multiple-cone SDPs. While GPU-based interior point SDP solvers have been deployed on supercomputers~\cite{fujisawa2012sc-extremely-sdp-interiorpoint}, all existing first-order SDP solvers are currently implemented on CPUs.

% \subsection{Graphics processing units (GPUs)}

==> sections/result.tex <==
%!TEX root = ../main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Results on the UW dataset
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table*}[t]
%     \centering
%     \caption{\textnormal{\bf Results on the UW dataset}.
%     \textnormal{We report the ATE, RPE and running time for Ceres, Manopt, and our proposed XM solver. The evaluation is conducted on four UW datasets with varying numbers of frames to demonstrate that our method is both fast and accurate across datasets of different scales. Ceres fails at a bad local minimum without a good initial guess, while Manopt performs significantly slower and even fails to solve within ten hours. To ensure practical usability, we limit the running time of our solver at 5 minutes; if this limit is exceeded, the solution is refined by Ceres.
%     }}
%     \label{tab:uw}
%     \begin{adjustbox}{width=\linewidth}
%     \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|}
%         \toprule
%         Datasets & \multicolumn{3}{c|}{UW-93\,(6033\,landmarks)} & \multicolumn{3}{c|}{UW-392\,(13902\,landmarks)} & \multicolumn{3}{c|}{UW-1934\,(67594\,landmarks)} & \multicolumn{3}{c|}{UW-10155\,(33782\,landmarks)} \\
%         \midrule
%         Metrics &\stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} &  \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R}  \\
%         \midrule\midrule
%         \textsc{Ceres} & \stackon{ $4.21$ }{ $0.06$ } & \stackon{ $0.18$ }{ $0.34$ } & \stackon{ 0.29 }{ 0.27 }& \stackon{ $23.31$ }{ 0.37 } & \stackon{ 0.43 }{ 0.41 } & \stackon{ 0.7 }{ 0.38 }& \stackon{ 227.15 }{ 3.85 } & \stackon{ 0.32 }{ 3.09 } & \stackon{ 0.63 }{ 0.55 }& \stackon{ 50.97 }{ 2.41 } & \stackon{ 0.71 }{ 1.47 } & \stackon{ 1.25 }{ 1.4 }\\
%         \midrule
%         Ceres-gt & \stackon{ 0.36 }{ 0.06 } & \stackon{ 0.0 }{ 0.0 } & \stackon{ 0.01 }{ 0.0 }& \stackon{ 3.59 }{ 0.36 } & \stackon{ 0.01 }{ 0.0 } & \stackon{ 0.01 }{ 0.0 }& \stackon{ 16.39 }{ 3.78 } & \stackon{ 0.01 }{ 0.0 } & \stackon{ 0.01 }{ 0.0 }& \stackon{ 21.49 }{ 2.4 } & \stackon{ 0.0 }{ 0.0 } & \stackon{ 0.0 }{ 0.0 }\\
%         \midrule
%         Ceres-gt-0.01& \stackon{ 11.61 }{ 0.06 } & \stackon{ 0.01 }{ 0.03 } & \stackon{ 0.02 }{ 0.05 }& \stackon{ 25.74 }{ 0.38 } & \stackon{ 0.04 }{ 0.08 } & \stackon{ 0.07 }{ 0.1 }& \stackon{ 427.79 }{ 3.73 } & \stackon{ 0.01 }{ 0.0 } & \stackon{ 0.01 }{ 0.0 }& \stackon{ 380.4 }{ 2.45 } & \stackon{ 0.04 }{ 0.05 } & \stackon{ 0.07 }{ 0.09 }\\
%         \midrule
%         Ceres-gt-0.1 & \stackon{ 9.24 }{ 0.06 } & \stackon{ 0.56 }{ 0.71 } & \stackon{ 1.01 }{ 0.6 }& \stackon{ 21.34 }{ 0.37 } & \stackon{ 0.37 }{ 0.39 } & \stackon{ 0.73 }{ 0.53 }& \stackon{ 70.43 }{ 3.76 } & \stackon{ 0.82 }{ 0.0 } & \stackon{ 1.3 }{ 0.16 }& \stackon{ 35.06 }{ 2.38 } & \stackon{ 0.33 }{ 0.36 } & \stackon{ 0.67 }{ 0.66 }\\
%         \midrule\midrule
%         Manopt  & \stackon{ 0.56 }{ 0.94 } & \stackon{ 0.0 }{ 0.0 } & \stackon{ 0.0 }{ 0.0 } & \stackon{ 21.43 }{  2.7 } & \stackon{ 0.0 }{ 0.0 } & \stackon{ 0.0 }{ 0.0 }& \stackon{ 236.46 }{ 69.15  } & \stackon{ 0.0 }{ 0.0 } & \stackon{ 0.01 }{ 0.0 }&\stackon{-}{336.76} &\stackon{-}{-} &\stackon{-}{-} \\
%         \midrule
%         \nameshort  & \stackon{ 0.07 }{ 0.94 } & \stackon{ 0.0 }{ 0.0 } & \stackon{ 0.0 }{ 0.0 } & \stackon{ 0.55 }{ 2.7 } & \stackon{ 0.0 }{ 0.0 } & \stackon{ 0.0 }{ 0.0 }& \stackon{ 2.09 }{ 69.15 } & \stackon{ 0.0 }{ 0.0 } & \stackon{ 0.01 }{ 0.0 }& \stackon{ 514.48 }{336.76} & \stackon{ 0.14 }{ 0.18 } & \stackon{ 0.31 }{ 0.31 }\\
%         \bottomrule
%     \end{tabular}
% \end{adjustbox}
% \end{table*}

\begin{table*}[t]
    \centering
    \caption{\textnormal{\bf Results on the UW dataset}.
    \textnormal{We report the ATE, RPE and running time for Ceres, Manopt, and our proposed \nameshort solver. The evaluation is conducted on four UW datasets with varying numbers of frames to demonstrate that our method is both fast and accurate across datasets of different scales. Ceres fails at a bad local minimum without a good initial guess, while Manopt performs significantly slower and even fails to solve within ten hours. 
    }}
    \label{tab:uw}
    \begin{adjustbox}{width=\linewidth}
        \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|}
            \toprule
            Datasets & \multicolumn{3}{c|}{UW-93\,(6033\,landmarks)} & \multicolumn{3}{c|}{UW-392\,(13902\,landmarks)} & \multicolumn{3}{c|}{UW-1934\,(67594\,landmarks)} & \multicolumn{3}{c|}{UW-10155\,(33782\,landmarks)} \\
            \midrule
            Metrics & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} &  \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R}  \\
            \midrule\midrule
            \textsc{Ceres} & \stackon{$4.21$}{$\bf 0.06$} & \stackon{$0.18$}{$19.47^{\circ}$} & \stackon{$0.29$}{$15.46^{\circ}$} & \stackon{$23.31$}{$0.37$} & \stackon{$0.43$}{$23.49^{\circ}$} & \stackon{$0.7$}{$21.80^{\circ}$} & \stackon{$227.15$}{$3.85$} & \stackon{$0.32$}{$177.20^{\circ}$} & \stackon{$0.63$}{$31.50^{\circ}$} & \stackon{$50.97$}{$2.41$} & \stackon{$0.71$}{$84.29^{\circ}$} & \stackon{$1.25$}{$80.19^{\circ}$} \\
            \midrule
            \textsc{Ceres-gt} & \stackon{$0.36$}{$0.06$} & \stackon{$\bf0.0$}{$\bf0.0^{\circ}$} & \stackon{$0.01$}{$\bf0.0^{\circ}$} & \stackon{$3.59$}{$\bf0.36$} & \stackon{$0.01$}{$\bf0.0^{\circ}$} & \stackon{$0.01$}{$\bf0.0^{\circ}$} & \stackon{$16.39$}{$3.78$} & \stackon{$0.01$}{$\bf0.0^{\circ}$} & \stackon{$\bf0.01$}{$\bf0.0^{\circ}$} & \stackon{$\bf21.49$}{$\bf2.4$} & \stackon{$\bf0.0$}{$\bf0.0^{\circ}$} & \stackon{$\bf0.0$}{$\bf0.0^{\circ}$} \\
            \midrule
            \textsc{Ceres-gt-0.01} & \stackon{$11.61$}{$0.06$} & \stackon{$0.01$}{$1.72^{\circ}$} & \stackon{$0.02$}{$2.87^{\circ}$} & \stackon{$25.74$}{$0.38$} & \stackon{$0.04$}{$4.58^{\circ}$} & \stackon{$0.07$}{$5.73^{\circ}$} & \stackon{$427.79$}{$\bf3.73$} & \stackon{$0.01$}{$\bf0.0^{\circ}$} & \stackon{$\bf0.01$}{$\bf0.0^{\circ}$} & \stackon{$380.4$}{$2.45$} & \stackon{$0.04$}{$2.87^{\circ}$} & \stackon{$0.07$}{$5.15^{\circ}$} \\
            \midrule
            \textsc{Ceres-gt-0.1} & \stackon{$9.24$}{$0.06$} & \stackon{$0.56$}{$40.29^{\circ}$} & \stackon{$1.01$}{$34.38^{\circ}$} & \stackon{$21.34$}{$0.37$} & \stackon{$0.37$}{$22.37^{\circ}$} & \stackon{$0.73$}{$30.38^{\circ}$} & \stackon{$70.43$}{$3.76$} & \stackon{$0.82$}{$\bf0.0^{\circ}$} & \stackon{$1.3$}{$9.17^{\circ}$} & \stackon{$35.06$}{$2.38$} & \stackon{$0.33$}{$20.57^{\circ}$} & \stackon{$0.67$}{$37.78^{\circ}$} \\
            \midrule\midrule
            \textsc{Manopt} & \stackon{$0.56$}{$0.94$} & \stackon{$\bf0.0$}{$\bf0.0^{\circ}$} & \stackon{$\bf0.0$}{$\bf0.0^{\circ}$} & \stackon{$21.43$}{$2.7$} & \stackon{$\bf0.0$}{$\bf0.0^{\circ}$} & \stackon{$\bf0.0$}{$\bf0.0^{\circ}$} & \stackon{$236.46$}{$69.15$} & \stackon{$\bf0.0$}{$\bf0.0^{\circ}$} & \stackon{$\bf0.01$}{$\bf0.0^{\circ}$} & \stackon{$**$}{$336.76$} & \stackon{$**$}{$**$} & \stackon{$**$}{$**$} \\
            \midrule
            \textsc{\nameshort} & \stackon{$\bf0.07$}{$0.94$} & \stackon{$\bf0.0$}{$\bf0.0^{\circ}$} & \stackon{$\bf0.0$}{$\bf0.0^{\circ}$} & \stackon{$\bf0.55$}{$2.7$} & \stackon{$\bf0.0$}{$\bf0.0^{\circ}$} & \stackon{$\bf0.0$}{$\bf0.0^{\circ}$} & \stackon{$\bf2.09$}{$69.15$} & \stackon{$\bf0.0$}{$\bf0.0^{\circ}$} & \stackon{$\bf0.01$}{$\bf0.0^{\circ}$} & \stackon{$ 4322.77 $}{$ 336.76$} & \stackon{$ 0.02 $}{$ 0.73 ^{\circ}$} & \stackon{$ 0.02 $}{$ 0.5 ^{\circ}$} \\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{table*}

\begin{table}[t]
    \centering
    \caption{\textnormal{\bf Results on the UW dataset (suboptimility and min-eig)}.
    \textnormal{We report the suboptimility gap and minimal eigen value of $Z$ matrix for our proposed \nameshort method. For large dataset we refer more on min-eig, because our estimation for suboptimility gap becomes huge. 
    }}
    \label{tab:uw-xm}
    \begin{adjustbox}{width=\linewidth}
    \begin{tabular}{l|c|c|c|c|}
        \toprule
        Datasets & \multicolumn{1}{c|}{UW-93} & \multicolumn{1}{c|}{UW-392} & \multicolumn{1}{c|}{UW-1934} & \multicolumn{1}{c|}{UW-10155} \\
        \midrule
        Suboptimility-Gap & $4.8 \times 10^{-4}$ & $4.2 \times 10^{-3}$ & $1.0 \times 10^{-2}$ & $6.2 \times 10^{5}$ \\
        \midrule
        Min-eig & $-8.8 \times 10^{-5}$ & $1.3 \times 10^{-7}$ & $1.2 \times 10^{-6}$ & $-2.1 \times 10^{1}$ \\

        \bottomrule
    \end{tabular}
\end{adjustbox}
\end{table}

% \begin{table*}[t]
%     \centering
%     \caption{\textnormal{\bf Results on the Replica dataset-median}.
%     \textnormal{
%     }}
%     \label{tab:replica-med}
%     \begin{adjustbox}{width=\linewidth}
%         \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%             \toprule
%             Datasets & \multicolumn{3}{c|}{\textsc{\nameshort}} & \multicolumn{3}{c|}{\textsc{\nameshort\,+\,reRANSAC\,+\,TEASER++}} & \multicolumn{3}{c|}{\textsc{\nameshort\,+\,Two-View\,Filter}} & \multicolumn{3}{c|}{\textsc{GLOMAP}}& \multicolumn{3}{c|}{\textsc{COLMAP}} \\
%             \midrule
%             Metrics & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} &  \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} & Total\,Time & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R}& Total\,Time & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R}  \\
%             \midrule\midrule
%             Room0-100 
%             & \stackon{$ 0.12 $}{$ 10.52 $} & \stackon{$ 0.005 $}{$ 0.323 ^{\circ}$} & \stackon{$ 0.007 $}{$ 0.083 ^{\circ}$}
%             & \stackon{$ 0.14 $}{$ 48.25 $} & \stackon{$ 0.005 $}{$ 0.758 ^{\circ}$} & \stackon{$ 0.008 $}{$ 0.079 ^{\circ}$}
%             & \stackon{$ 0.12 $}{$ 13.71 $} & \stackon{$ 0.005 $}{$ 1.025 ^{\circ}$} & \stackon{$ 0.008 $}{$ 0.077 ^{\circ}$}
%             & $ 45.97 $ & \stackon{$ 0.003 $}{$ 0.469 ^{\circ}$} & \stackon{$ 0.004 $}{$ 0.05 ^{\circ}$}\\
%             \midrule
%             Room-2000
%             & \stackon{$ 8.5 $}{$ 1142.74 $} & \stackon{$ 0.012 $}{$ 1.38 ^{\circ}$} & \stackon{$ 0.017 $}{$ 0.44 ^{\circ}$}
%             &$**$&$**$&$**$
%             & \stackon{$ 16.26 $}{$ 1868.24 $} & \stackon{$ 0.003 $}{$ 0.379 ^{\circ}$} & \stackon{$ 0.005 $}{$ 0.242 ^{\circ}$}
%             & $ 6329.29 $ & \stackon{$ 0.001 $}{$ 0.136 ^{\circ}$} & \stackon{$ 0.001 $}{$ 0.043 ^{\circ}$}\\
%             \midrule\midrule
%             Room1-100 
%             & \stackon{$ 0.14 $}{$ 13.08 $} & \stackon{$ 0.009 $}{$ 1.847 ^{\circ}$} & \stackon{$ 0.013 $}{$ 0.16 ^{\circ}$}
%             & \stackon{$ 0.15 $}{$ 73.95 $} & \stackon{$ 0.007 $}{$ 1.504 ^{\circ}$} & \stackon{$ 0.012 $}{$ 0.177 ^{\circ}$}
%             &  \stackon{$ 0.14 $}{$ 16.19 $} & \stackon{$ 0.01 $}{$ 2.056 ^{\circ}$} & \stackon{$ 0.014 $}{$ 0.176 ^{\circ}$}
%             & $ 62.7 $ & \stackon{$ 0.014 $}{$ 1.409 ^{\circ}$} & \stackon{$ 0.019 $}{$ 0.122 ^{\circ}$}\\
%             \midrule
%             Room1-2000
%             & \stackon{$ 7.37 $}{$ 1156.6 $} & \stackon{$ 0.102 $}{$ 10.57 ^{\circ}$} & \stackon{$ 0.135 $}{$ 8.971 ^{\circ}$}
%             &$**$&$**$&$**$
%             & \stackon{$ 6.18 $}{$ 1651.12 $} & \stackon{$ 0.005 $}{$ 0.428 ^{\circ}$} & \stackon{$ 0.008 $}{$ 0.418 ^{\circ}$}
%             & $ 4717.94 $ & \stackon{$ 0.001 $}{$ 0.166 ^{\circ}$} & \stackon{$ 0.002 $}{$ 0.066 ^{\circ}$}\\
%             \midrule\midrule
%             Office0-100 
%             & \stackon{$ 0.15 $}{$ 12.75 $} & \stackon{$ 0.04 $}{$ 3.554 ^{\circ}$} & \stackon{$ 0.051 $}{$ 0.128 ^{\circ}$}
%             & \stackon{$ 0.13 $}{$ 59.47 $} & \stackon{$ 0.019 $}{$ 1.243 ^{\circ}$} & \stackon{$ 0.025 $}{$ 0.122 ^{\circ}$}
%             & \stackon{$ 0.12 $}{$ 16.53 $} & \stackon{$ 0.024 $}{$ 3.385 ^{\circ}$} & \stackon{$ 0.033 $}{$ 0.127 ^{\circ}$}
%             & $ 36.66 $ & \stackon{$ 0.015 $}{$ 0.559 ^{\circ}$} & \stackon{$ 0.019 $}{$ 0.04 ^{\circ}$}\\
%             \midrule
%             Office0-2000
%             & \stackon{$ 4.6 $}{$ 730.15 $} & \stackon{$ 0.249 $}{$ 9.423 ^{\circ}$} & \stackon{$ 0.322 $}{$ 12.713 ^{\circ}$}
%             &$**$&$**$&$**$
%             & \stackon{$ 5.61 $}{$ 1181.42 $} & \stackon{$ 0.061 $}{$ 3.353 ^{\circ}$} & \stackon{$ 0.079 $}{$ 3.294 ^{\circ}$}
%             & $ 3855.62 $ & \stackon{$ 0.024 $}{$ 2.822 ^{\circ}$} & \stackon{$ 0.034 $}{$ 0.058 ^{\circ}$}\\
%             \midrule\midrule
%             Office1-100 
%             & \stackon{$ 0.13 $}{$ 8.13 $} & \stackon{$ 0.022 $}{$ 2.708 ^{\circ}$} & \stackon{$ 0.03 $}{$ 0.2 ^{\circ}$}
%             & \stackon{$ 0.15 $}{$ 31.72 $} & \stackon{$ 0.016 $}{$ 1.326 ^{\circ}$} & \stackon{$ 0.023 $}{$ 0.147 ^{\circ}$}
%             & \stackon{$ 0.15 $}{$ 10.81 $} & \stackon{$ 0.015 $}{$ 2.032 ^{\circ}$} & \stackon{$ 0.023 $}{$ 0.138 ^{\circ}$}
%             & $23.07$ & \stackon{$ 0.006 $}{$ 1.423 ^{\circ}$} & \stackon{$ 0.008 $}{$ 0.021 ^{\circ}$}\\
%             \midrule
%             Office1-2000
%             & \stackon{$ 23.1 $}{$ 759.43 $} & \stackon{$ 0.049 $}{$ 2.997 ^{\circ}$} & \stackon{$ 0.064 $}{$ 2.623 ^{\circ}$}
%             &$**$&$**$&$**$
%             & \stackon{$ 20.72 $}{$ 1285.34 $} & \stackon{$ 0.08 $}{$ 9.95 ^{\circ}$} & \stackon{$ 0.104 $}{$ 3.404 ^{\circ}$}
%             & $ 3976.75 $ & \stackon{$ 0.642 $}{$ 55.545 ^{\circ}$} & \stackon{$ 0.672 $}{$ 2.626 ^{\circ}$}
%             \\
%             \bottomrule
%         \end{tabular}
%     \end{adjustbox}
% \end{table*} 

% \begin{table*}[t]
%     \centering
%     \caption{\textnormal{\bf Results on the Replica dataset-median}.}
%     \label{tab:replica-med1}
%     \begin{adjustbox}{width=\linewidth}
%         \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|}
%             \toprule
%             Datasets & \multicolumn{3}{c|}{\textsc{\nameshort}} & \multicolumn{3}{c|}{\textsc{\nameshort\,+\,Two-View\,Filter}} & \multicolumn{3}{c|}{\textsc{GLOMAP}} & \multicolumn{3}{c|}{\textsc{COLMAP}} \\
%             \midrule
%             Metrics & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} & Total\,Time & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} & Total\,Time & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} \\
%             \midrule\midrule
%             Room0-100 
%             & \stackon{$ 0.12 $}{$ 10.52 $} & \stackon{$ 0.005 $}{$ 0.323 ^{\circ}$} & \stackon{$ 0.007 $}{$ 0.083 ^{\circ}$}
%             & \stackon{$ 0.12 $}{$ 13.71 $} & \stackon{$ 0.005 $}{$ 1.025 ^{\circ}$} & \stackon{$ 0.008 $}{$ 0.077 ^{\circ}$}
%             & $ 45.97 $ & \stackon{$ 0.003 $}{$ 0.469 ^{\circ}$} & \stackon{$ 0.004 $}{$ 0.05 ^{\circ}$} 
%             & $ 102.32 $ & \stackon{$ 0.003 $}{$ 0.582 ^{\circ}$} & \stackon{$ 0.004 $}{$ 0.038 ^{\circ}$}\\
%             \midrule
%             Room-2000
%             & \stackon{$ 8.5 $}{$ 1142.74 $} & \stackon{$ 0.012 $}{$ 1.38 ^{\circ}$} & \stackon{$ 0.017 $}{$ 0.44 ^{\circ}$}
%             & \stackon{$ 16.26 $}{$ 1868.24 $} & \stackon{$ 0.003 $}{$ 0.379 ^{\circ}$} & \stackon{$ 0.005 $}{$ 0.242 ^{\circ}$}
%             & \stackon{$ 349.77 + 607.54 $}{$ 6329.29 - 349.77 - 607.54$} & \stackon{$ 0.001 $}{$ 0.136 ^{\circ}$} & \stackon{$ 0.001 $}{$ 0.043 ^{\circ}$} 
%             & $ \stackon{$ 74827.56 $}{$ 160.02 $} $ & \stackon{$ 0.001 $}{$ 0.078 ^{\circ}$} & \stackon{$ 0.001 $}{$ 0.068 ^{\circ}$}\\
%             \midrule\midrule
%             Room1-100 
%             & \stackon{$ 0.14 $}{$ 13.08 $} & \stackon{$ 0.009 $}{$ 1.847 ^{\circ}$} & \stackon{$ 0.013 $}{$ 0.16 ^{\circ}$}
%             & \stackon{$ 0.14 $}{$ 16.19 $} & \stackon{$ 0.01 $}{$ 2.056 ^{\circ}$} & \stackon{$ 0.014 $}{$ 0.176 ^{\circ}$}
%             & $ 62.7 $ & \stackon{$ 0.014 $}{$ 1.409 ^{\circ}$} & \stackon{$ 0.019 $}{$ 0.122 ^{\circ}$} 
%             & $ 146.38 $ & \stackon{$ 0.06 $}{$ 10.765 ^{\circ}$} & \stackon{$ 0.072 $}{$ 0.726 ^{\circ}$}\\
%             \midrule
%             Room1-2000
%             & \stackon{$ 7.37 $}{$ 1156.6 $} & \stackon{$ 0.102 $}{$ 10.57 ^{\circ}$} & \stackon{$ 0.135 $}{$ 8.971 ^{\circ}$}
%             & \stackon{$ 6.18 $}{$ 1651.12 $} & \stackon{$ 0.005 $}{$ 0.428 ^{\circ}$} & \stackon{$ 0.008 $}{$ 0.418 ^{\circ}$}
%             & \stackon{$ 379.45 531.55 $}{$ 4717.94 - 379.45 531.55$} & \stackon{$ 0.001 $}{$ 0.166 ^{\circ}$} & \stackon{$ 0.002 $}{$ 0.066 ^{\circ}$} \\
%             \midrule\midrule
%             Office0-100 
%             & \stackon{$ 0.15 $}{$ 12.75 $} & \stackon{$ 0.04 $}{$ 3.554 ^{\circ}$} & \stackon{$ 0.051 $}{$ 0.128 ^{\circ}$}
%             & \stackon{$ 0.12 $}{$ 16.53 $} & \stackon{$ 0.024 $}{$ 3.385 ^{\circ}$} & \stackon{$ 0.033 $}{$ 0.127 ^{\circ}$}
%             & $ 36.66 $ & \stackon{$ 0.015 $}{$ 0.559 ^{\circ}$} & \stackon{$ 0.019 $}{$ 0.04 ^{\circ}$} \\
%             \midrule
%             Office0-2000
%             & \stackon{$ 4.6 $}{$ 730.15 $} & \stackon{$ 0.249 $}{$ 9.423 ^{\circ}$} & \stackon{$ 0.322 $}{$ 12.713 ^{\circ}$}
%             & \stackon{$ 5.61 $}{$ 1181.42 $} & \stackon{$ 0.061 $}{$ 3.353 ^{\circ}$} & \stackon{$ 0.079 $}{$ 3.294 ^{\circ}$}
%             & \stackon{$ 168.36 445.49 $}{$ 3855.62 - 168.36 445.49 $} & \stackon{$ 0.024 $}{$ 2.822 ^{\circ}$} & \stackon{$ 0.034 $}{$ 0.058 ^{\circ}$} \\
%             \midrule\midrule
%             Office1-100 
%             & \stackon{$ 0.13 $}{$ 8.13 $} & \stackon{$ 0.022 $}{$ 2.708 ^{\circ}$} & \stackon{$ 0.03 $}{$ 0.2 ^{\circ}$}
%             & \stackon{$ 0.15 $}{$ 10.81 $} & \stackon{$ 0.015 $}{$ 2.032 ^{\circ}$} & \stackon{$ 0.023 $}{$ 0.138 ^{\circ}$}
%             & $23.07$ & \stackon{$ 0.006 $}{$ 1.423 ^{\circ}$} & \stackon{$ 0.008 $}{$ 0.021 ^{\circ}$} \\
%             \midrule
%             Office1-2000
%             & \stackon{$ 23.1 $}{$ 759.43 $} & \stackon{$ 0.049 $}{$ 2.997 ^{\circ}$} & \stackon{$ 0.064 $}{$ 2.623 ^{\circ}$}
%             & \stackon{$ 20.72 $}{$ 1285.34 $} & \stackon{$ 0.08 $}{$ 9.95 ^{\circ}$} & \stackon{$ 0.104 $}{$ 3.404 ^{\circ}$}
%             & \stackon{$ 140.53 525.81 $}{$ 3976.75 - 140.53 525.81$} & \stackon{$ 0.642 $}{$ 55.545 ^{\circ}$} & \stackon{$ 0.672 $}{$ 2.626 ^{\circ}$} \\
%             \bottomrule
%         \end{tabular}
%     \end{adjustbox}
% \end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Results on the Replica dataset-median
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[t]
    \centering
    \caption{\textnormal{\bf Results on the Replica dataset-median}.}
    \label{tab:replica}
    \begin{adjustbox}{width=\linewidth}
        \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|}
            \toprule
            Datasets & \multicolumn{3}{c|}{\textsc{\xmdouble}} & \multicolumn{3}{c|}{\textsc{\xmdouble + Filter}} & \multicolumn{3}{c|}{\glomap} & \multicolumn{3}{c|}{\colmap} \\
            \midrule
            Metrics & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} \\
            \midrule\midrule
            Room0-100 
            & \stackon{$ 0.12 $}{$ 10.52 $} & \stackon{$ 0.005 $}{$ 0.323 ^{\circ}$} & \stackon{$ 0.007 $}{$ 0.083 ^{\circ}$}
            & \stackon{$ 0.12 $}{$ 13.71 $} & \stackon{$ 0.005 $}{$ 1.025 ^{\circ}$} & \stackon{$ 0.008 $}{$ 0.077 ^{\circ}$}
            & \stackon{$ 39.57 $}{$ 6.4 $} & \stackon{$ 0.003 $}{$ 0.469 ^{\circ}$} & \stackon{$ 0.004 $}{$ 0.05 ^{\circ}$} 
            & \stackon{$ 100.61 $}{$ 1.71 $}& \stackon{$ 0.003 $}{$ 0.582 ^{\circ}$} & \stackon{$ 0.004 $}{$ 0.038 ^{\circ}$}\\
            \midrule
            Room0-2000
            & \stackon{$ 8.5 $}{$ 1142.74 $} & \stackon{$ 0.012 $}{$ 1.38 ^{\circ}$} & \stackon{$ 0.017 $}{$ 0.44 ^{\circ}$}
            & \stackon{$ 16.26 $}{$ 1868.24 $} & \stackon{$ 0.003 $}{$ 0.379 ^{\circ}$} & \stackon{$ 0.005 $}{$ 0.242 ^{\circ}$}
            & \stackon{$ 5371.98 $}{$ 957.31 $} & \stackon{$ 0.001 $}{$ 0.136 ^{\circ}$} & \stackon{$ 0.001 $}{$ 0.043 ^{\circ}$} 
            & \stackon{$ 74827.56 $}{$ 120.02 $} & \stackon{$ 0.001 $}{$ 0.078 ^{\circ}$} & \stackon{$ 0.001 $}{$ 0.068 ^{\circ}$}\\
            \midrule\midrule
            Room1-100 
            & \stackon{$ 0.14 $}{$ 13.08 $} & \stackon{$ 0.009 $}{$ 1.847 ^{\circ}$} & \stackon{$ 0.013 $}{$ 0.16 ^{\circ}$}
            & \stackon{$ 0.14 $}{$ 16.19 $} & \stackon{$ 0.01 $}{$ 2.056 ^{\circ}$} & \stackon{$ 0.014 $}{$ 0.176 ^{\circ}$}
            & \stackon{$ 53.95 $}{$ 8.75 $} & \stackon{$ 0.014 $}{$ 1.409 ^{\circ}$} & \stackon{$ 0.019 $}{$ 0.122 ^{\circ}$} 
            & \stackon{$ 144.39 $}{$ 1.99 $} & \stackon{$ 0.06 $}{$ 10.765 ^{\circ}$} & \stackon{$ 0.072 $}{$ 0.726 ^{\circ}$}\\
            \midrule
            Room1-2000
            & \stackon{$ 7.37 $}{$ 1156.6 $} & \stackon{$ 0.102 $}{$ 10.57 ^{\circ}$} & \stackon{$ 0.135 $}{$ 8.971 ^{\circ}$}
            & \stackon{$ 6.18 $}{$ 1651.12 $} & \stackon{$ 0.005 $}{$ 0.428 ^{\circ}$} & \stackon{$ 0.008 $}{$ 0.418 ^{\circ}$}
            & \stackon{$ 3806.94 $}{$ 911.0 $} & \stackon{$ 0.001 $}{$ 0.166 ^{\circ}$} & \stackon{$ 0.002 $}{$ 0.066 ^{\circ}$} 
            & \stackon{$ 64912.5 $}{$ 379.45 $} & \stackon{$ 0.002 $}{$ 0.156 ^{\circ}$} & \stackon{$ 0.002 $}{$ 0.06 ^{\circ}$}\\
            \midrule\midrule
            Office0-100 
            & \stackon{$ 0.15 $}{$ 12.75 $} & \stackon{$ 0.04 $}{$ 3.554 ^{\circ}$} & \stackon{$ 0.051 $}{$ 0.128 ^{\circ}$}
            & \stackon{$ 0.12 $}{$ 16.53 $} & \stackon{$ 0.024 $}{$ 3.385 ^{\circ}$} & \stackon{$ 0.033 $}{$ 0.127 ^{\circ}$}
            & \stackon{$ 27.99 $ }{$ 8.67 $}& \stackon{$ 0.015 $}{$ 0.559 ^{\circ}$} & \stackon{$ 0.019 $}{$ 0.04 ^{\circ}$} 
            & \stackon{$ 49.02 $}{$ 3.58 $ }& \stackon{$ 0.019 $}{$ 1.53 ^{\circ}$} & \stackon{$ 0.028 $}{$ 0.067 ^{\circ}$}\\
            \midrule
            Office0-2000
            & \stackon{$ 4.6 $}{$ 730.15 $} & \stackon{$ 0.249 $}{$ 9.423 ^{\circ}$} & \stackon{$ 0.322 $}{$ 12.713 ^{\circ}$}
            & \stackon{$ 5.61 $}{$ 1181.42 $} & \stackon{$ 0.061 $}{$ 3.353 ^{\circ}$} & \stackon{$ 0.079 $}{$ 3.294 ^{\circ}$}
            & \stackon{$ 3241.77 $}{$ 613.85 $} & \stackon{$ 0.024 $}{$ 2.822 ^{\circ}$} & \stackon{$ 0.034 $}{$ 0.058 ^{\circ}$} 
            & \stackon{$ 35682.24 $}{$ 168.36 $} & \stackon{$ 0.003 $}{$ 0.184 ^{\circ}$} & \stackon{$ 0.004 $}{$ 0.06 ^{\circ}$}\\
            \midrule\midrule
            Office1-100 
            & \stackon{$ 0.13 $}{$ 8.13 $} & \stackon{$ 0.022 $}{$ 2.708 ^{\circ}$} & \stackon{$ 0.03 $}{$ 0.2 ^{\circ}$}
            & \stackon{$ 0.15 $}{$ 10.81 $} & \stackon{$ 0.015 $}{$ 2.032 ^{\circ}$} & \stackon{$ 0.023 $}{$ 0.138 ^{\circ}$}
            & \stackon{$ 18.7 $}{$ 4.37 $}& \stackon{$ 0.006 $}{$ 1.423 ^{\circ}$} & \stackon{$ 0.008 $}{$ 0.021 ^{\circ}$} 
            & \stackon{$ 61.5 $}{$ 1.36$ }& \stackon{$ 0.014 $}{$ 3.366 ^{\circ}$} & \stackon{$ 0.021 $}{$ 0.039 ^{\circ}$}\\
            \midrule
            Office1-2000
            & \stackon{$ 23.1 $}{$ 759.43 $} & \stackon{$ 0.049 $}{$ 2.997 ^{\circ}$} & \stackon{$ 0.064 $}{$ 2.623 ^{\circ}$}
            & \stackon{$ 230.25 $}{$ 1270.29 $} & \stackon{$ 0.038 $}{$ 5.08 ^{\circ}$} & \stackon{$ 0.052 $}{$ 1.643 ^{\circ}$}
            & \stackon{$ 3310.41 $}{$ 666.34 $} & \stackon{$ 0.642 $}{$ 55.545 ^{\circ}$} & \stackon{$ 0.672 $}{$ 2.626 ^{\circ}$} 
            &\stackon{$ 25512.84 $}{$ 140.53 $} & \stackon{$ 0.078 $}{$ 13.882 ^{\circ}$} & \stackon{$ 0.112 $}{$ 0.157 ^{\circ}$}\\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{table*}

\begin{table}[t]
    \centering
    \caption{\textnormal{\bf Results on the Replica dataset (min-eig and suboptimility)}.
    \textnormal{We report the minimal eigen value of $Z$ matrix for our proposed \nameshort method. Here because we add relularity term, suboptimility gap is not a good measure. 
    }}
    \label{tab:rep-xm}
    \begin{adjustbox}{width=\linewidth}
        \begin{tabular}{l|c|c|c|c|}
            \toprule
            Method & \multicolumn{2}{c|}{\xmdouble} & \multicolumn{2}{c|}{\xmdouble-F} \\
            \midrule
            Metric & Min-eig & Suboptimility-gap &  Min-eig & Suboptimility-gap\\
            \midrule\midrule
            Room0-100 & $1.1\times10^{-5}$ & $1.9\times10^{-6}$ & $1.1\times10^{-5}$& $7.4\times10^{-8}$\\
            \midrule
            Room0-2000 & $3.5\times10^{-8}$ &$2.2\times10^{-5}$ & $-6.3\times10^{-8}$ &$5.9\times10^{-6}$\\
            \midrule
            Room1-100 & $2.6\times10^{-6}$ & $7.9\times10^{-4}$ & $1.3\times10^{-5}$ &$1.8\times10^{-6}$\\
            \midrule
            Room1-2000 & $5.8\times10^{-8}$ & $2.2\times10^{-4}$ & $-4.6\times10^{-7}$ &$4.5\times10^{-6}$\\
            \midrule
            office0-100 & $-8.0\times10^{-7}$ & $1.4\times10^{-7}$ & $-1.0\times10^{-6}$ &$1.1\times10^{-7}$\\
            \midrule
            office0-2000 & $4.7\times10^{-7}$ & $5.2\times10^{-4}$ & $-1.5\times10^{-6}$ &$6.7\times10^{-6}$\\
            \midrule
            office1-100 & $-8.0\times10^{-7}$ & $1.0\times10^{-7}$ & $8.5\times10^{-7}$ &$2.4\times10^{-8}$\\
            \midrule
            office1-2000 & $-4.2\times10^{-8}$ & $2.3\times10^{-5}$ & $6.8\times10^{-8}$ &$3.8\times10^{-4}$\\
            \midrule
            \bottomrule
        \end{tabular}        
\end{adjustbox}
\end{table}

\begin{adjustbox}{width=0.9\linewidth}
    \begin{tikzpicture}
        % 数据表扩展到12行
        \pgfplotstableread{
            Label  Match Index  Depth Filter Matrix Solver
            R1     0 0 0 0 0 0
            R2     0 0 0 0 0 0
            R3     0 0 0 0 0 0
            R4     0 0 0 0 0 0
            R5     0 0 0 0 0 0
            A1     349.77 607.54 55.16 0 130.26 8.5
            A2     379.45 531.55 63.0 0 182.6 7.37
            A3     168.36 445.49 40.72 0 75.59 4.6
            A4     140.53 525.81 40.98 0 52.12 23.1
            A5     0       0      0     0      0     0
            B1     349.77 607.54 53.63 727.3 130.0 16.26
            B2     379.45 531.55 63.7 511.36 165.06 6.18
            B3     168.36 445.49 43.41 480.9 71.59 5.61
            B4     140.53 525.81 37.18 543.33 52.36 20.72
            B5     0       0      0         0     0         0
        }\testdata



        \begin{axis}[
            ybar stacked,
            ymin=0,
            ymax=2000,
            xtick={1,6,11},  % 每个簇的中心点
            xticklabels={\,, \xmdouble, \xmdouble-F}, % 每簇共享的标签
            legend style={cells={anchor=west}, legend pos=north west, font = \scriptsize},
            bar width=10pt, % 控制柱子宽度
            enlarge x limits=0.1, % 调整簇间距
            reverse legend=true,
        ]

        % 绘制数据
        \addplot [fill=green!80] 
            table [x expr=\coordindex, y=Match] 
            {\testdata};
        \addlegendentry{Match}
    
        \addplot [fill=blue!60] 
            table [x expr=\coordindex, y=Index]
             {\testdata};
        \addlegendentry{Index}
    
        \addplot [fill=purple!60] 
            table [x expr=\coordindex, y=Depth]
            {\testdata};
        \addlegendentry{Depth}

        \addplot [fill=orange!60] 
            table [x expr=\coordindex, y=Filter] {\testdata};
        \addlegendentry{Filter}

        \addplot [fill=yellow!60] 
            table [x expr=\coordindex, y=Matrix] {\testdata};
        \addlegendentry{Matrix}

        \addplot [fill=red!60] 
        table [x expr=\coordindex, y=Solver] {\testdata};
        \addlegendentry{Solver}
    
        \end{axis}
    \end{tikzpicture}
\end{adjustbox}

\begin{adjustbox}{width= 0.8\linewidth}
    \begin{tikzpicture}
        % 数据表扩展到12行
        \pgfplotstableread{
Label  Match   Index  Depth Filter Matrix Solver
R1     0 0 0 0 0 0
R2     0 0 0 0 0 0
R3     0 0 0 0 0 0
R4     0 0 0 0 0 0
R5     0 0 0 0 0 0
A1     1.71 4.69 1.57 0 2.54 0.12
A2     1.99 6.76 1.62 0 2.71 0.14
A3     3.58 5.09 1.53 0 2.55 0.15
A4     1.36 3.01 1.52 0 2.32 0.13
A5     0       0      0     0      0     0 
% B1     1.71 4.69 5.38 1.6 32.43 0 2.62
% B2     1.99 6.76 5.83 1.62 54.71 0 2.85
% B3     3.58 5.09 5.15 1.53 41.7 0 2.41
% B4     1.36 3.01 5.41 1.55 18.22 0 2.22
% B5     0       0      0         0  0     0        0
C1     1.71 4.69 1.6 3.34 2.58 0.12
C2     1.99 6.76 1.6 3.21 2.62 0.14
C3     3.58 5.09 1.56 3.49 2.81 0.12
C4     1.36 3.01 1.52 2.8 2.41 0.15
C5     0       0      0         0     0  0        
}\testdata



        \begin{axis}[
            ybar stacked,
            ymin=0,
            ymax=20,
            xtick={1, 6, 11},  % 每个簇的中心点
            xticklabels={\,,\xmdouble, \xmdouble-F}, % 每簇共享的标签
            legend style={cells={anchor=west}, legend pos=north west, font = \scriptsize},
            bar width=10pt, % 控制柱子宽度
            enlarge x limits=0.1, % 调整簇间距
            reverse legend=true,
        ]

         % 绘制数据
         \addplot [fill=green!80] 
         table [x expr=\coordindex, y=Match] 
         {\testdata};
     \addlegendentry{Match}
 
     \addplot [fill=blue!60] 
         table [x expr=\coordindex, y=Index]
          {\testdata};
     \addlegendentry{Index}
 
     \addplot [fill=purple!60] 
         table [x expr=\coordindex, y=Depth]
         {\testdata};
     \addlegendentry{Depth}

     \addplot [fill=orange!60] 
         table [x expr=\coordindex, y=Filter] {\testdata};
     \addlegendentry{Filter}

     \addplot [fill=yellow!60] 
         table [x expr=\coordindex, y=Matrix] {\testdata};
     \addlegendentry{Matrix}

     \addplot [fill=red!60] 
     table [x expr=\coordindex, y=Solver] {\testdata};
     \addlegendentry{Solver}
    
        \end{axis}
    \end{tikzpicture}
\end{adjustbox}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Results on the MIP NERF
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table*}[t]
%     \centering
%     \caption{\textnormal{\bf pre-Results on the Mip-Nerf}.}
%     \label{tab:mipnerf_pre}
%     \begin{adjustbox}{width=\linewidth}
%         \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|}
%             \toprule
%             Datasets &\multicolumn{3}{c|}{\xmdouble + \ceres}& \multicolumn{3}{c|}{\textsc{\xmdouble + Filter + \ceres}} & \multicolumn{3}{c|}{\textsc{\xmdouble + Filter + \teaserpp} + \ceres} &\multicolumn{3}{c|}{\xmdouble  + Filter + \teaserpp + re\ransac + \ceres}\\
%             \midrule
%             Metrics & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} & \stackon{Solver\,Time}{Processing\,
%             Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} \\
%             \midrule\midrule
%             Kitchen
%             & \stackon{$ 1.05 $}{$ 216.03 $} & \stackon{$ 0.013 $}{$ 0.11 ^{\circ}$} & \stackon{$ 0.018 $}{$ 0.143 ^{\circ}$}
%             & \stackon{$ 1.09 $}{$ 227.9 $} & \stackon{$ 0.01 $}{$ 0.089 ^{\circ}$} & \stackon{$ 0.014 $}{$ 0.118 ^{\circ}$}
%             & \stackon{$ 1.07 $}{$ 307.02 $} & \stackon{$ 0.007 $}{$ 0.055 ^{\circ}$} & \stackon{$ 0.011 $}{$ 0.089 ^{\circ}$}
%             & \stackon{$ 1.48 $}{$ 216.48 $} & \stackon{$ 0.003 $}{$ 0.04 ^{\circ}$} & \stackon{$ 0.004 $}{$ 0.05 ^{\circ}$}\\
%             \midrule
%             garden
%             & \stackon{$ 0.57 $}{$ 168.29 $} & \stackon{$ 0.002 $}{$ 0.016 ^{\circ}$} & \stackon{$ 0.002 $}{$ 0.018 ^{\circ}$}
%             & \stackon{$ 0.58 $}{$ 176.29 $} & \stackon{$ 0.003 $}{$ 0.029 ^{\circ}$} & \stackon{$ 0.004 $}{$ 0.017 ^{\circ}$}
%             & \stackon{$ 0.61 $}{$ 208.49 $} & \stackon{$ 0.002 $}{$ 0.016 ^{\circ}$} & \stackon{$ 0.002 $}{$ 0.018 ^{\circ}$}
%             & \stackon{$ 0.72 $}{$ 493.66 $} & \stackon{$ 0.002 $}{$ 0.014 ^{\circ}$} & \stackon{$ 0.002 $}{$ 0.014 ^{\circ}$}\\
%             \midrule
%             bicycle
%             & \stackon{$ 0.76 $}{$ 147.79 $} & \stackon{$ 0.01 $}{$ 0.15 ^{\circ}$} & \stackon{$ 0.013 $}{$ 0.044 ^{\circ}$}
%             & \stackon{$ 0.76 $}{$ 149.38 $} & \stackon{$ 0.01 $}{$ 0.138 ^{\circ}$} & \stackon{$ 0.015 $}{$ 0.081 ^{\circ}$}
%             & \stackon{$ 0.81 $}{$ 157.36 $} & \stackon{$ 0.018 $}{$ 0.275 ^{\circ}$} & \stackon{$ 0.026 $}{$ 0.18 ^{\circ}$}
%             & \stackon{$ 0.7 $}{$ 344.93 $} & \stackon{$ 0.021 $}{$ 0.332 ^{\circ}$} & \stackon{$ 0.027 $}{$ 0.093 ^{\circ}$}\\
%             \midrule
%             Room
%             & \stackon{$ 1.01 $}{$ 187.6 $} & \stackon{$ 0.004 $}{$ 0.101 ^{\circ}$} & \stackon{$ 0.005 $}{$ 0.144 ^{\circ}$}
%             & \stackon{$ 0.86 $}{$ 201.21 $} & \stackon{$ 0.003 $}{$ 0.088 ^{\circ}$} & \stackon{$ 0.004 $}{$ 0.13 ^{\circ}$}
%             & \stackon{$ 0.87 $}{$ 264.81 $} & \stackon{$ 0.002 $}{$ 0.066 ^{\circ}$} & \stackon{$ 0.003 $}{$ 0.099 ^{\circ}$}
%             & \stackon{$ 0.92 $}{$ 1340.28 $} & \stackon{$ 0.002 $}{$ 0.067 ^{\circ}$} & \stackon{$ 0.003 $}{$ 0.106 ^{\circ}$}
            
%             \\
%             \bottomrule
%         \end{tabular}
%     \end{adjustbox}
% \end{table*}

\begin{table*}[t]
    \centering
    \caption{\textnormal{\bf Results on the Mip-Nerf}.}
    \label{tab:mipnerf}
    \begin{adjustbox}{width=\linewidth}
        \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|}
            \toprule
            Datasets & \multicolumn{3}{c|}{\textsc{Filter + \xmdouble}} & \multicolumn{3}{c|}{\textsc{Filter + \xmdouble + Ceres}}& \multicolumn{3}{c|}{\glomap} & \multicolumn{3}{c|}{\colmap}  \\
            \midrule
            Metrics & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} \\
            \midrule\midrule
            Kitchen
            & \stackon{$ 0.8 $}{$ 229.4 $} & \stackon{$ 0.203 $}{$ 2.341 ^{\circ}$} & \stackon{$ 0.296 $}{$ 2.91 ^{\circ}$}
            & \stackon{$ 19.99 $}{$ 229.82 $} & \stackon{$ 0.018 $}{$ 0.154 ^{\circ}$} & \stackon{$ 0.027 $}{$ 0.201 ^{\circ}$}
            & \stackon{$ 363.22 $}{$124.23$} & \stackon{$ 0.016 $}{$ 0.107 ^{\circ}$} & \stackon{$ 0.023 $}{$ 0.135 ^{\circ}$}
            & \stackon{$1422.96$}{$97.26$} & \stackon{$0.0$}{$0.0^{\circ}$} & \stackon{$0.0$}{$0.0^{\circ}$}
            \\
            \midrule
            garden
            & \stackon{$ 0.65 $}{$ 174.26 $} & \stackon{$ 0.318 $}{$ 1.6 ^{\circ}$} & \stackon{$ 0.463 $}{$ 1.501 ^{\circ}$}
            & \stackon{$ 4.63 $}{$ 174.57 $} & \stackon{$ 0.002 $}{$ 0.021 ^{\circ}$} & \stackon{$ 0.003 $}{$ 0.025 ^{\circ}$}
            & \stackon{$ 193.86 $}{$ 90.7 $}  & \stackon{$ 0.013 $}{$ 0.061 ^{\circ}$} & \stackon{$ 0.02 $}{$ 0.067 ^{\circ}$}
            & \stackon{$486.84$}{$78.1$} & \stackon{$0.0$}{$0.0^{\circ}$} & \stackon{$0.0$}{$0.0^{\circ}$}
            \\
            \midrule
            bicycle
            & \stackon{$ 0.58 $}{$ 144.84 $} & \stackon{$ 1.235 $}{$ 9.989 ^{\circ}$} & \stackon{$ 2.182 $}{$ 4.799 ^{\circ}$}
            & \stackon{$ 23.05 $}{$ 145.75 $} & \stackon{$ 0.019 $}{$ 0.229 ^{\circ}$} & \stackon{$ 0.028 $}{$ 0.219 ^{\circ}$}
            & \stackon{$ 77.76 $}{$ 79.84 $} & \stackon{$ 0.039 $}{$ 0.51 ^{\circ}$} & \stackon{$ 0.056 $}{$ 0.114 ^{\circ}$}
            & \stackon{$273.84$}{$75.16$} & \stackon{$0.0$}{$0.0^{\circ}$} & \stackon{$0.0$}{$0.0^{\circ}$}
            \\
            \midrule
            Room
            & \stackon{$ 1.01 $}{$ 197.38 $} & \stackon{$ 0.184 $}{$ 4.181 ^{\circ}$} & \stackon{$ 0.253 $}{$ 3.41 ^{\circ}$}
            & \stackon{$ 25.36 $}{$ 223.44 $} & \stackon{$ 0.002 $}{$ 0.06 ^{\circ}$} & \stackon{$ 0.002 $}{$ 0.084 ^{\circ}$}
            & \stackon{$ 269.39 $}{$ 96.26 $} & \stackon{$ 0.003 $}{$ 0.083 ^{\circ}$} & \stackon{$ 0.003 $}{$ 0.029 ^{\circ}$}
            & \stackon{$958.5$}{$62.47$} & \stackon{$0.0$}{$0.0^{\circ}$} & \stackon{$0.0$}{$0.0^{\circ}$}
            \\
            \midrule
            Alameda
            & \stackon{$ 280.13 $}{$ 3348.46 $} & \stackon{$ 0.009 $}{$ 0.317 ^{\circ}$} & \stackon{$ 0.014 $}{$ 0.493 ^{\circ}$}\\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{table*}

\begin{table}[t]
    \centering
    \caption{\textnormal{\bf Results on the MipNerf dataset (min-eig and suboptimility)}.
    \textnormal{We report the minimal eigenvalue of the $Z$ matrix for our proposed \nameshort method. Here because we add a regularity term, the suboptimality gap is not a good measure. 
    }}
    \label{tab:rep-xm}
    \begin{adjustbox}{width=\linewidth}
        \begin{tabular}{l|c|c|c|c|c|}
            \toprule
            Metric & kitchen & garden & bicycle & room & alameda \\
            \midrule
            Min-eig & $1.1\times10^{-10}$ & $-3.6\times10^{-9}$ & $4.8\times10^{-8}$ & $-4.6\times10^{-7}$ & $-3.8\times10^{-7}$ \\
            \midrule
            Suboptimility-gap & $8.9\times10^{-8}$ & $8.8\times10^{-9}$ & $2.5\times10^{-5}$ & $4.5\times10^{-6}$ & $8.1\times10^{-2}$ \\
            \bottomrule
        \end{tabular}        
    \end{adjustbox}
\end{table}


\begin{table}[t]
    \centering
    \caption{\textnormal{\bf Results on the Mip-Nerf}.}
    \label{tab:mipnerf}
    \begin{adjustbox}{width=\linewidth}
        \begin{tabular}{l|l|l|l|l|l|l|}
            \toprule
            \multirow{3}{*}{Method} & \multirow{3}{*}{Metrics} & \multicolumn{5}{c|}{Datasets} \\
            \cmidrule{3-7}
            & & \stackon{-187865}{Kitchen-279} & \stackon{-106858}{Garden-185} & \stackon{-41866}{Bicycle-194} & \stackon{-111783}{Room-311} & \stackon{-416665}{Alameda-1724} \\
            \midrule
            \multirow{6}{*}{\textsc{xm}}
            & \stackon{(\nameshort + \ceres)}{Solver Time} & \stackon{$19.19$}{$0.8~+ $} & \stackon{$3.98 $}{$0.65~+ $} & \stackon{$22.47$}{$0.58~+ $} & \stackon{$24.35$}{$1.01~+ $} & \stackon{$218.13$}{$62.0~+ $} \\
            \cmidrule{2-7}
            & Processing Time & $229.82$ & $174.57$ & $145.75$ & $223.44$ & $3348.46$ \\
            \cmidrule{2-7}
            & ATE-T & $0.018$ & $0.002$ & $0.019$ & $0.002$ & $0.009$ \\
            & ATE-R & $0.154^\circ$ & $0.021^\circ$ & $0.229^\circ$ & $0.06^\circ$ & $0.317^\circ$ \\
            \cmidrule{2-7}
            & RPE-T & $0.027$ & $0.003$ & $0.028$ & $0.002$ & $0.014$ \\
            & RPE-R & $0.201^\circ$ & $0.025^\circ$ & $0.219^\circ$ & $0.084^\circ$ & $0.493^\circ$ \\
            \midrule
            \multirow{6}{*}{\textsc{glomap}}
            & Solver Time & $363.22$ & $193.86$ & $77.76$ & $269.39$ & $1169.83$ \\
            \cmidrule{2-7}
            & Processing Time & $124.23$ & $90.7$ & $79.84$ & $96.26$ & $2631.69$ \\
            \cmidrule{2-7}
            & ATE-T & $0.016$ & $0.013$ & $0.039$ & $0.003$ & $0.001$ \\
            & ATE-R & $0.107^\circ$ & $0.061^\circ$ & $0.51^\circ$ & $0.083^\circ$ & $0.074^\circ$ \\
            \cmidrule{2-7}
            & RPE-T & $0.023$ & $0.02$ & $0.056$ & $0.003$ & $0.002$ \\
            & RPE-R & $0.135^\circ$ & $0.067^\circ$ & $0.114^\circ$ & $0.029^\circ$ & $0.053^\circ$ \\
            \midrule
            \multirow{6}{*}{\textsc{colmap}}
            & Solver Time & $1422.96$ & $486.84$ & $273.84$ & $958.5$ &\\
            \cmidrule{2-7}
            & Processing Time & $97.26$ & $78.1$ & $75.16$ & $62.47$ &  \\
            \cmidrule{2-7}
            & ATE-T & $0.0$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\
            & ATE-R & $0.0^\circ$ & $0.0^\circ$ & $0.0^\circ$ & $0.0^\circ$ & $0.0^\circ$ \\
            \cmidrule{2-7}
            & RPE-T & $0.0$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\
            & RPE-R & $0.0^\circ$ & $0.0^\circ$ & $0.0^\circ$ & $0.0^\circ$ & $0.0^\circ$ \\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{table}

% \begin{table}[t]
%     \centering
%     \caption{\textnormal{\bf Results on the MipNerf dataset (min-eig and suboptimility)}.
%     \textnormal{We report the minimal eigen value of $Z$ matrix for our proposed \nameshort method. Here because we add relularity term, suboptimility gap is not a good measure. 
%     }}
%     \label{tab:rep-xm}
%     \begin{adjustbox}{width=\linewidth}
%         \begin{tabular}{l|c|c|c|c|}
%             \toprule
%             Method & \multicolumn{2}{c|}{Filter + \xmdouble} & \multicolumn{2}{c|}{Filter + \xmdouble + Ceres} \\
%             \midrule
%             Metric & Min-eig & Suboptimility-gap &  Min-eig & Suboptimility-gap\\
%             \midrule\midrule
%             kitchen & $-9.8\times10^{-10}$ & $1.4\times10^{-7}$ & $1.1\times10^{-10}$& $8.9\times10^{-8}$\\
%             \midrule
%             garden & $-2.9\times10^{-9}$ &$3.1\times10^{-7}$ & $-3.6\times10^{-9}$ &$8.8\times10^{-9}$\\
%             \midrule
%             bicycle & $1.7\times10^{-8}$ & $8.9\times10^{-6}$ & $4.8\times10^{-8}$ &$2.5\times10^{-5}$\\
%             \midrule
%             room & $5.8\times10^{-8}$ & $2.2\times10^{-4}$ & $-4.6\times10^{-7}$ &$4.5\times10^{-6}$\\
%             \midrule
%             alameda & $-8.0\times10^{-7}$ & $1.0\times10^{-7}$ & $-3.8\times10^{-7}$ &$8.1\times10^{-2}$\\
%             \bottomrule
%         \end{tabular}        
% \end{adjustbox}
% \end{table}

\begin{adjustbox}{width=0.9\linewidth}
    \begin{tikzpicture}
        % 数据表扩展到12行
        \pgfplotstableread{
            Label  Match Index  Depth Filter Matrix XM Ceres
            R1     0 0 0 0 0 0 0
            % R4     0 0 0 0 0 0
            % R5     0 0 0 0 0 0
            % A1     87.65 36.58 55.49 16.33 33.36 0.8
            % A2     53.77 37.93 55.47 8.58 18.51 0.65
            % A3     56.23 23.99 54.64 2.18 7.8 0.58
            % A4     61.77 34.49 59.55 18.91 22.65 1.01
            % A5     0       0      0     0      0     0
            B1     87.65 36.58 55.22 16.06 30.66 0.8 19.19
            B2     53.77 37.93 59.62 8.8 14.46 0.65 3.98
            B3     56.23 23.99 50.69 2.17 12.67 0.58 22.47
            B4     61.77 34.49 59.5 18.72 24.6 1.01 24.35
            B5     2494.29 137.69 283.46 90.45 342.57 62.0 218.13
        }\testdata


        \begin{axis}[
            ybar stacked,
            ymin=0,
            ymax=300,
            xtick={1,2,3,4,5},  % 每个簇的中心点
            xticklabels={Kitchen,Garden,Bicycle,Room,Alameda}, % 每簇共享的标签
            legend style={cells={anchor=west}, legend pos=north west, font = \scriptsize},
            bar width=10pt, % 控制柱子宽度
            enlarge x limits=0.1, % 调整簇间距
            reverse legend=true,
        ]

        % 绘制数据
        \addplot [fill=green!80] 
            table [x expr=\coordindex, y=Match] 
            {\testdata};
        \addlegendentry{Match}
    
        \addplot [fill=blue!60] 
            table [x expr=\coordindex, y=Index]
             {\testdata};
        \addlegendentry{Index}
    
        \addplot [fill=purple!60] 
            table [x expr=\coordindex, y=Depth]
            {\testdata};
        \addlegendentry{Depth}

        \addplot [fill=orange!60] 
            table [x expr=\coordindex, y=Filter] {\testdata};
        \addlegendentry{Filter}

        \addplot [fill=yellow!60] 
            table [x expr=\coordindex, y=Matrix] {\testdata};
        \addlegendentry{Matrix}

        \addplot [fill=red!60] 
        table [x expr=\coordindex, y=XM] {\testdata};
        \addlegendentry{XM}

        \addplot [fill=pink!60] 
        table [x expr=\coordindex, y=Ceres] {\testdata};
        \addlegendentry{Ceres}
    
    
        \end{axis}
    \end{tikzpicture}
\end{adjustbox}


% \begin{table*}[t]
%     \centering
%     \caption{\textnormal{\bf Results on the Replica dataset}.
%     \textnormal{
%     }}
%     \label{tab:replica}
%     \begin{adjustbox}{width=\linewidth}
%         \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%             \toprule
%             Datasets & \multicolumn{3}{c|}{\textsc{\nameshort}} & \multicolumn{3}{c|}{\textsc{\nameshort\,+\,reRANSAC\,+\,TEASER++}} & \multicolumn{3}{c|}{\textsc{\nameshort\,+\,Two-View\,Filter}} & \multicolumn{3}{c|}{\textsc{GLOMAP}}& \multicolumn{3}{c|}{\textsc{COLMAP}} \\
%             \midrule
%             Metrics & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} &  \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} & Total\,Time & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R}& Total\,Time & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R}  \\
%             \midrule\midrule
%             Room0-100 
%             & \stackon{$ 0.13 $}{$ 10.58 $} & \stackon{$ 0.005 $}{$ 0.321 ^{\circ}$} & \stackon{$ 0.008 $}{$ 0.094 ^{\circ}$}
%             & \stackon{$ 0.14 $}{$ 48.17 $} & \stackon{$ 0.006 $}{$ 0.76 ^{\circ}$} & \stackon{$ 0.008 $}{$ 0.087 ^{\circ}$}
%             & \stackon{$ 0.13 $}{$ 13.97 $} & \stackon{$ 0.007 $}{$ 1.545 ^{\circ}$} & \stackon{$ 0.01 $}{$ 0.1 ^{\circ}$}
%             & $ 45.97 $ & \stackon{$ 0.003 $}{$ 0.484 ^{\circ}$} & \stackon{$ 0.004 $}{$ 0.056 ^{\circ}$}\\
%             \midrule
%             Room-2000
%             & \stackon{$ 8.5 $}{$ 1142.74 $} & \stackon{$ 0.013 $}{$ 1.194 ^{\circ}$} & \stackon{$ 0.018 $}{$ 0.621 ^{\circ}$}
%             &$**$&$**$&$**$
%             & \stackon{$ 16.26 $}{$ 1868.24 $} & \stackon{$ 0.004 $}{$ 0.44 ^{\circ}$} & \stackon{$ 0.006 $}{$ 0.26 ^{\circ}$}
%             & $ 6329.29 $ & \stackon{$ 0.001 $}{$ 0.13 ^{\circ}$} & \stackon{$ 0.001 $}{$ 0.044 ^{\circ}$}\\
%             \midrule\midrule
%             Room1-100 
%             & \stackon{$ 0.14 $}{$ 13.08 $} & \stackon{$ 0.009 $}{$ 1.847 ^{\circ}$} & \stackon{$ 0.013 $}{$ 0.168 ^{\circ}$}
%             & \stackon{$ 0.15 $}{$ 73.74 $} & \stackon{$ 0.009 $}{$ 1.955 ^{\circ}$} & \stackon{$ 0.013 $}{$ 0.192 ^{\circ}$}
%             & \stackon{$ 0.14 $}{$ 16.06 $} & \stackon{$ 0.01 $}{$ 2.077 ^{\circ}$} & \stackon{$ 0.014 $}{$ 0.188 ^{\circ}$}
%             & $ 62.7 $ & \stackon{$ 0.014 $}{$ 1.428 ^{\circ}$} & \stackon{$ 0.019 $}{$ 0.141 ^{\circ}$}\\
%             \midrule
%             Room1-2000
%             & \stackon{$ 7.37 $}{$ 1156.6 $} & \stackon{$ 0.102 $}{$ 10.57 ^{\circ}$} & \stackon{$ 0.135 $}{$ 8.971 ^{\circ}$}
%             &$**$&$**$&$**$
%             & \stackon{$ 6.18 $}{$ 1651.12 $} & \stackon{$ 0.006 $}{$ 0.472 ^{\circ}$} & \stackon{$ 0.009 $}{$ 0.415 ^{\circ}$}
%             & $ 4717.94 $ & \stackon{$ 0.201 $}{$ 0.218 ^{\circ}$} & \stackon{$ 0.403 $}{$ 0.189 ^{\circ}$}\\
%             \midrule\midrule
%             Office0-100 
%             & \stackon{$ 0.16 $}{$ 13.23 $} & \stackon{$ 0.039 $}{$ 3.475 ^{\circ}$} & \stackon{$ 0.053 $}{$ 0.213 ^{\circ}$}
%             & \stackon{$ 0.14 $}{$ 59.55 $} & \stackon{$ 0.024 $}{$ 1.828 ^{\circ}$} & \stackon{$ 0.032 $}{$ 0.132 ^{\circ}$}
%             & \stackon{$ 0.13 $}{$ 16.32 $} & \stackon{$ 0.025 $}{$ 3.265 ^{\circ}$} & \stackon{$ 0.035 $}{$ 0.142 ^{\circ}$}
%             & $ 36.66 $ & \stackon{$ 0.015 $}{$ 0.558 ^{\circ}$} & \stackon{$ 0.021 $}{$ 0.039 ^{\circ}$}\\
%             \midrule
%             Office0-2000
%             & \stackon{$ 4.6 $}{$ 730.15 $} & \stackon{$ 0.263 $}{$ 11.734 ^{\circ}$} & \stackon{$ 0.351 $}{$ 14.791 ^{\circ}$}
%             &$**$&$**$&$**$
%             & \stackon{$ 5.55 $}{$ 1209.75 $} & \stackon{$ 0.06 $}{$ 3.327 ^{\circ}$} & \stackon{$ 0.083 $}{$ 3.61 ^{\circ}$}
%             & $ 3855.62 $ & \stackon{$ 1.603 $}{$ 3.035 ^{\circ}$} & \stackon{$ 3.135 $}{$ 0.536 ^{\circ}$}\\
%             \midrule\midrule
%             Office1-100 
%             & \stackon{$ 0.13 $}{$ 8.21 $} & \stackon{$ 0.023 $}{$ 2.723 ^{\circ}$} & \stackon{$ 0.031 $}{$ 0.219 ^{\circ}$}
%             & \stackon{$ 0.15 $}{$ 31.72 $} & \stackon{$ 0.016 $}{$ 1.326 ^{\circ}$} & \stackon{$ 0.023 $}{$ 0.147 ^{\circ}$}
%             & \stackon{$ 0.13 $}{$ 11.1 $} & \stackon{$ 0.017 $}{$ 3.181 ^{\circ}$} & \stackon{$ 0.024 $}{$ 0.135 ^{\circ}$}
%             & $ 23.07 $ & \stackon{$ 0.006 $}{$ 1.424 ^{\circ}$} & \stackon{$ 0.009 $}{$ 0.023 ^{\circ}$}\\
%             \midrule
%             Office1-2000
%             & \stackon{$ 23.1 $}{$ 759.43 $} & \stackon{$ 0.049 $}{$ 2.997 ^{\circ}$} & \stackon{$ 0.064 $}{$ 2.623 ^{\circ}$}
%             &$**$&$**$&$**$
%             & \stackon{$ 20.72 $}{$ 1285.34 $} & \stackon{$ 0.08 $}{$ 9.982 ^{\circ}$} & \stackon{$ 0.109 $}{$ 3.789 ^{\circ}$}
%             \\
%             \bottomrule
%         \end{tabular}
%     \end{adjustbox}
% \end{table*}    

% \begin{table}[t]
%     \centering
%     \caption{\textnormal{\bf Results on the Replica dataset (min-eig)}.
%     \textnormal{We report the minimal eigen value of $Z$ matrix for our proposed \nameshort method. Here because we add relularity term, suboptimility gap is not a good measure. 
%     }}
%     \label{tab:rep-xm}
%     \begin{adjustbox}{width=\linewidth}
%         \begin{tabular}{l|c|c|c|c|}
%             \toprule
%             Method & \nameshort & \nameshort-T & \nameshort-F \\
%             \midrule
%             Room0-100 & $1.1\times10^{-5}$/uu & $5.1\times10^{-6}$ & $1.1\times10^{-5}$ \\
%             Room0-2000 & $3.5\times10^{-8}$ & $**$ & $-6.3\times10^{-8}$ \\
%             Room1-100 & $2.6\times10^{-6}$ & $1.3\times10^{-7}$ & $1.3\times10^{-5}$ \\
%             Room1-2000 & $5.8\times10^{-8}$ & $**$ & $-4.6\times10^{-7}$ \\
%             office0-100 & $-8.0\times10^{-7}$ & $-1.7\times10^{-6}$ & $-1.0\times10^{-6}$ \\
%             office0-2000 & $4.7\times10^{-7}$ & $**$ & $-1.5\times10^{-6}$ \\
%             office1-100 & $-8.0\times10^{-7}$ & $-1.5\times10^{-5}$ & $8.5\times10^{-7}$ \\
%             \bottomrule
%         \end{tabular}        
% \end{adjustbox}
% \end{table}

\begin{table}[t]
    \centering
    \caption{\textnormal{\bf Results on the IMC2023}.}
    \label{tab:imc}
    \begin{adjustbox}{width=\linewidth}
        \begin{tabular}{l|c|c|c|c|c|c|}
            \toprule
            Datasets & \multicolumn{3}{c|}{\textsc{Filter + \xmdouble + Ceres}}& \multicolumn{3}{c|}{\glomap}   \\
            \midrule
            Metrics & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R}  \\
            \midrule\midrule
            \stackon{-203244}{Rome-2063}
            & \stackon{$ 19.17 + 300.16 $}{$ 4877.89 $} & \stackon{$ 0.011 $}{$ 0.96 ^{\circ}$} & \stackon{$ 0.018 $}{$ 1.226 ^{\circ}$}
            & \stackon{$ 9813.04 $}{$3459.04$} & \stackon{$ 0.003 $}{$ 0.09 ^{\circ}$} & \stackon{$ 0.005 $}{$ 0.069 ^{\circ}$}
            \\
            \midrule
            \stackon{-62561}{Gate-1363}
            & \stackon{$ 2.92 + 99.66 $}{$ 1349.74 $} & \stackon{$ 0.038 $}{$ 1.329 ^{\circ}$} & \stackon{$ 0.089 $}{$ 2.022 ^{\circ}$}
            & \stackon{$ 2263.79 $}{$712.56$} & \stackon{$ 0.018 $}{$ 0.41 ^{\circ}$} & \stackon{$ 0.047 $}{$ 0.19 ^{\circ}$}
            \\
            \midrule
            \stackon{-78026}{Temple-904}
            & \stackon{$ 1.34 + 93.5 $}{$ 1026.65 $} & \stackon{$ 0.011 $}{$ 0.817 ^{\circ}$} & \stackon{$ 0.02 $}{$ 0.437 ^{\circ}$}
            & \stackon{$ 1560.86 $}{$600.4$} & \stackon{$ 0.012 $}{$ 0.276 ^{\circ}$} & \stackon{$ 0.03 $}{$ 0.216 ^{\circ}$}
            \\
            \midrule
            \stackon{-314422}{Paris-3765}
            & \stackon{$ 22.17 + 304.49 $}{$ 16645.16 $} & \stackon{$ 0.008 $}{$ 0.473 ^{\circ}$} & \stackon{$ 0.017 $}{$ 0.561 ^{\circ}$}
            & \stackon{$ 74560.1 $}{$10598.8$} & \stackon{$ 0.009 $}{$ 0.117 ^{\circ}$} & \stackon{$ 0.017 $}{$ 0.087 ^{\circ}$}
            \\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{table}

\begin{table}[t]
    \centering
    \caption{\textnormal{\bf Results on the C3VD}.}
    \label{tab:imc}
    \begin{adjustbox}{width=\linewidth}
        \begin{tabular}{l|c|c|c|}
            \toprule
            Datasets & \multicolumn{3}{c|}{\textsc{Filter + \xmdouble + Ceres}}\\
            \midrule
            Metrics & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} \\
            \midrule\midrule
            medical1
            & \stackon{$ 0.76 + 33.81 $}{$ 155.77 $} & \stackon{$ 0.086 $}{$ 25.609 ^{\circ}$} & \stackon{$ 0.115 $}{$ 3.404 ^{\circ}$}
            \\
            \midrule
            medical2
            & \stackon{$ 0.72 + 70.33 $}{$ 261.18 $} & \stackon{$ 0.142 $}{$ 155.465 ^{\circ}$} & \stackon{$ 0.184 $}{$ 3.978 ^{\circ}$}
            \\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{table}






==> tables/c3vddataset.tex <==
\begin{table}[t]
    \centering
    \caption{\textnormal{\bf Results on C3VD}.}
    \label{tab:imc}
    \begin{adjustbox}{width=\linewidth}
        \begin{tabular}{l|c|c|c|c|c|c|c|c|c}
            \toprule
            Datasets & \multicolumn{3}{c|}{\textsc{Filter + \xmdouble + GT-depth}} & \multicolumn{3}{c|}{\textsc{Filter + \xmdouble}}& \multicolumn{3}{c|}{\glomap}\\
            \midrule
            Metrics & \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R}& \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R}& \stackon{Solver\,Time}{Processing\,Time} & \stackon{ATE-T}{ATE-R} & \stackon{RPE-T}{RPE-R} \\
            \midrule\midrule
            medical5
            & \stackon{$ 0.31 + 0 $}{$ 55.45 $} & \stackon{$ 0.009 $}{$ 3.284 ^{\circ}$} & \stackon{$ 0.015 $}{$ 0.647 ^{\circ}$}
            & \stackon{$ 0.34 + 0 $}{$ 30.19 $} & \stackon{$ 0.109 $}{$ 11.64 ^{\circ}$} & \stackon{$ 0.169 $}{$ 3.191 ^{\circ}$}
            & $ 101.22 $ & \stackon{$ 0.013 $}{$ 2.24 ^{\circ}$} & \stackon{$ 0.018 $}{$ 0.28 ^{\circ}$}
            \\
            \midrule
            medical6
            & \stackon{$ 0.46 + 0 $}{$ 171.35 $} & \stackon{$ 0.014 $}{$ 4.102 ^{\circ}$} & \stackon{$ 0.019 $}{$ 0.851 ^{\circ}$}
            & \stackon{$ 0.47 + 0 $}{$ 166.19 $} & \stackon{$ 0.262 $}{$ 116.79 ^{\circ}$} & \stackon{$ 0.352 $}{$ 4.729 ^{\circ}$}
            & $ 371.67 $ & \stackon{$ 0.013 $}{$ 1.001 ^{\circ}$} & \stackon{$ 0.019 $}{$ 0.373 ^{\circ}$}
            \\
            \midrule
            medical7
            & \stackon{$ 0.81 + 0 $}{$ 261.58 $} & \stackon{$ 0.01 $}{$ 3.69 ^{\circ}$} & \stackon{$ 0.013 $}{$ 1.231 ^{\circ}$}
            & \stackon{$ 0.89 + 0 $}{$ 250.48 $} & \stackon{$ 0.047 $}{$ 131.686 ^{\circ}$} & \stackon{$ 0.062 $}{$ 3.564 ^{\circ}$}
            & $ 719.42 $ & \stackon{$ 0.019 $}{$ 10.305 ^{\circ}$} & \stackon{$ 0.028 $}{$ 0.931 ^{\circ}$}
            \\
            \midrule
            medical8
            & \stackon{$ 0.23 + 0 $}{$ 56.84 $} & \stackon{$ 0.72 $}{$ 66.107 ^{\circ}$} & \stackon{$ 1.196 $}{$ 0.062 ^{\circ}$}
            & \stackon{$ 0.22 + 0 $}{$ 38.25 $} & \stackon{$ 0.452 $}{$ 159.909 ^{\circ}$} & \stackon{$ 0.704 $}{$ 0.091 ^{\circ}$}
            & $ 513.57 $ & \stackon{$ 0.005 $}{$ 30.806 ^{\circ}$} & \stackon{$ 0.034 $}{$ 0.188 ^{\circ}$}
            \\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
    \vspace{-8mm}
\end{table}

==> tables/conversion_speed.tex <==
%!TEX root = ../main.tex

\begin{table}[t]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        & \yalmip (Matlab) & \sostools (Matlab) & \tssos (Julia) & Ours (Matlab) \\
        \hline
        $N = 4$ & $8.18$s & $3.39$s & $2.40$s & $\bm{0.09}$\textbf{s} \\
        \hline 
        $N = 30$ & $68.89$s & $>30$min & $2.51$s & $\bm{0.32}$\textbf{s}  \\
        \hline
    \end{tabular}
    \vspace{1mm}
    \caption{POP-SDP conversion time of $4$ conversion packages in the inverted pendulum problem. When $N = 30$, \sostools takes more than $30$ miniutes and takes more than $300$GB memory.
    \label{tab:exp:gen:conversion-speed}}
\end{table}

==> tables/hyper_params.tex <==
%!TEX root = ../main.tex

\begin{table}[t]
    \label{tab:exp:gen:hyper-params}
    \centering
    \resizebox{\columnwidth}{!} {
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
        \hline
        & $d_x$ & $d_u$ & $\text{deg}_{\max}$ & $N$ & $\text{size}(M)$ & $\#M$ & $\text{size}(L)$ & $\#L$ & $m_{\text{SDP}}$ & $\log_{10}\xi$ \\
        \hline 
        Inverted Pendulum & $4$ & $1$ & $2$ & $30$ & $55$ & $30$ & $10$ & $60$ & $47351$ & $\bm{-2.58}$ ($\bm{-2.93}$) \\
        \hline 
        Cart-Pole & $5$ & $1$ & $2$ & $30$ & $105$ & $30$ & $14$ & $273$ & $168961$ & $\bm{-2.89}$ ($\bm{-2.98}$) \\
        \hline 
        Car Back-in & $4 (+3)$ & $4$ & $3$ & $30$  & $190$ & $30$ & $19$ & $659$ & $509141$ & $\bm{-1.87}$ ($\bm{-1.99}$) \\
        \hline 
        Vehicle Landing & $8$ & $2$ & $2$ & $50$ & $190$ & $50$ & $19$ & $499$ & $946326$ & $\bm{-2.47}$ ($\bm{-2.42}$) \\
        \hline 
        Flying Robot & $8$ & $4$ & $2$ & $60$ & $231$ & $60$ & $21$ & $659$ & $1595001$ & $\bm{-2.57}$ ($\bm{-2.49}$) \\
        \hline 
    \end{tabular}
    }

    \caption{Hyper-parameters and suboptimality gaps in five numerical experiments. Means (medians) are reported for suboptimality gaps from \cuadmm. In the car back-in case, $(+3)$ denotes the $(A,B,C)$ parameters in the separation line.}
\end{table}

==> tables/timing.tex <==
%!TEX root = ../main.tex

\begin{table}[t]
    \label{tab:exp:gen:timing}
    \centering
    \resizebox{\columnwidth}{!} {
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
        \multirow{2}{*}{} & \multicolumn{4}{c|}{Per-Iteration Cost} & \multicolumn{4}{c|}{Total Time} \\
        \cline{2-9}
        & \mosek & \cdcs & \sdpnal & \cuadmm & \mosek & \cdcs & \sdpnal & \cuadmm \\
        \hline 
        \multirow{2}{*}{Inverted Pendulum} & \multirow{2}{*}{$0.5$s} & \multirow{2}{*}{$11.1$ms} & \multirow{2}{*}{$59.1$ms} & \multirow{2}{*}{\textbf{$\bm{8.9}$ms}} & \multirow{2}{*}{$9.5$s} & \multirow{2}{*}{$110.3$s} & \multirow{2}{*}{$264.4$s} & $31.2$s ($14.6$s) \\
        \cline{9-9} 
        & & & & & & & & \textbf{$\bm{0.66}$s} (\textbf{$\bm{0.62}$s}) \\
        \hline
        Cart-Pole & $7.5$s & $147.1$ms & $588.2$ms & \textbf{$\bm{29.1}$ms} & \textbf{$\bm{112.0}$s} & $1471$s & $3671$s & $183.0$s ($173.1$s) \\
        \hline 
        Car Back-in & $778.1$s & $612.3$ms & $1.8$s & $\bm{44.8}$\textbf{ms} & $>5$h & $6123$s & $>5$h & \textbf{$\bm{431.5}$s} (\textbf{$\bm{536.8}$s})  \\
        \hline 
        Vehicle Landing & $1387$s & $1.0$s & $2.4$s & $\bm{118.3}$\textbf{ms} & $>5$h & $2.9$h & $>5$h &  \textbf{$\bm{919.2}$s} (\textbf{$\bm{1165}$s}) \\
        \hline 
        Flying Robot & - & $1.7$s & $6.2$s & $\bm{169.7}$\textbf{ms} & - & $>5$h & $>5$h & \textbf{$\bm{1648}$s} (\textbf{$\bm{2027}$s}) \\
        \hline 
    \end{tabular}
    }

    \caption{Per-interation costs and total time costs for different solvers across five experiments. For \cuadmm, we report the means (medians) of total time costs. The pendulum case lists total time costs with (upper) and without (lower) warm starts. For the flying robot case, \MOSEK runs out of 1TB memory.}
\end{table}
